Learning to Play Table Tennis From Scratch using Muscular Robots

Dynamic tasks like table tennis are relatively easy to learn for humans but pose significant challenges to robots. Such tasks require accurate control of fast movements and precise timing in the presence of imprecise state estimation of the flying ball and the robot. Reinforcement Learning (RL) has shown promise in learning of complex control tasks from data. However, applying step-based RL to dynamic tasks on real systems is safety-critical as RL requires exploring and failing safely for millions of time steps in high-speed regimes. In this paper, we demonstrate that safe learning of table tennis using model-free Reinforcement Learning can be achieved by using robot arms driven by pneumatic artificial muscles (PAMs). Softness and back-drivability properties of PAMs prevent the system from leaving the safe region of its state space. In this manner, RL empowers the robot to return and smash real balls with 5 m\s and 12m\s on average to a desired landing point. Our setup allows the agent to learn this safety-critical task (i) without safety constraints in the algorithm, (ii) while maximizing the speed of returned balls directly in the reward function (iii) using a stochastic policy that acts directly on the low-level controls of the real system and (iv) trains for thousands of trials (v) from scratch without any prior knowledge. Additionally, we present HYSR, a practical hybrid sim and real training that avoids playing real balls during training by randomly replaying recorded ball trajectories in simulation and applying actions to the real robot. This work is the first to (a) fail-safe learn of a safety-critical dynamic task using anthropomorphic robot arms, (b) learn a precision-demanding problem with a PAM-driven system despite the control challenges and (c) train robots to play table tennis without real balls. Videos and datasets are available at muscularTT.embodied.ml.

==> figures/video/hit.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
axis on top,
xmin=0.5,
xmax=1920.5,
xlabel style={font=\color{white!15!black}},
xlabel={hit},
y dir=reverse,
ymin=0.5,
ymax=1080.5,
axis background/.style={fill=white},
ylabel near ticks,
xlabel near ticks,
legend style={at={(.6,.45)},anchor=north west,legend cell align=left,align=left,fill=none,draw=none}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=1920.5, ymin=0.5, ymax=1080.5] {./hit-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/video/initPosture.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
axis on top,
xmin=0.5,
xmax=1920.5,
xlabel style={font=\color{white!15!black}},
xlabel={inital posture},
y dir=reverse,
ymin=0.5,
ymax=1080.5,
axis background/.style={fill=white},
ylabel near ticks,
xlabel near ticks,
legend style={at={(.6,.45)},anchor=north west,legend cell align=left,align=left,fill=none,draw=none}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=1920.5, ymin=0.5, ymax=1080.5] {./initPosture-1.png};
\end{axis}
\end{tikzpicture}%

==> figures/video/prep.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figwidth,
height=\figheight,
at={(0\figwidth,0\figheight)},
scale only axis,
axis on top,
xmin=0.5,
xmax=1920.5,
xlabel style={font=\color{white!15!black}},
xlabel={preparation},
y dir=reverse,
ymin=0.5,
ymax=1080.5,
axis background/.style={fill=white},
ylabel near ticks,
xlabel near ticks,
legend style={at={(.6,.45)},anchor=north west,legend cell align=left,align=left,fill=none,draw=none}
]
\addplot [forget plot] graphics [xmin=0.5, xmax=1920.5, ymin=0.5, ymax=1080.5] {./prep-1.png};
\end{axis}
\end{tikzpicture}%
